Leveraging Explicit Reasoning for Inference Integration in Commonsense-Augmented Dialogue Models

Open-domain dialogue systems need to grasp social commonsense to understand and respond effectively to human users. Commonsense-augmented dialogue models have been proposed that aim to infer commonsense knowledge from dialogue contexts in order to improve response quality. However, existing approaches to commonsense-augmented dialogue rely on implicit reasoning to integrate commonsense inferences during response generation. In this study, we explore the impact of explicit reasoning against implicit reasoning over commonsense for dialogue response generation. Our findings demonstrate that separating commonsense reasoning into explicit steps for generating, selecting, and integrating commonsense into responses leads to better dialogue interactions, improving naturalness, engagement, specificity, and overall quality. Subsequent analyses of these findings unveil insights into the effectiveness of various types of commonsense in generating responses and the particular response traits enhanced through explicit reasoning for commonsense integration. Our work advances research in open-domain dialogue by achieving a new state-of-the-art in commonsense-augmented response generation.

==> section/acknowledgments.tex <==
\section*{Acknowledgments}

We gratefully acknowledge the support of Amazon for this work. Any opinions, findings, and conclusions or recommendations expressed in this material are those of the authors and do not necessarily reflect the views of Amazon.

==> section/old/impact-of-commonsensetype-all-metrics.tex <==
% \begin{figure*}[htb]
%     \centering
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/natural_by_cstype.pdf}
%         \caption{Naturalness}
%         \label{fig:sub1}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/engaging_by_cstype.pdf}
%         \caption{Engagingness}
%         \label{fig:sub2}
%     \end{subfigure}
    
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/specific_by_cstype.pdf}
%         \caption{Specificity}
%         \label{fig:sub3}
%     \end{subfigure}
%     \hfill
%     \begin{subfigure}{0.49\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{img/quality_by_cstype.pdf}
%         \caption{Overall Quality}
%         \label{fig:sub4}
%     \end{subfigure}
%     \caption{Proportion of wins by \caps{Crest-e} against other models, based on the type of commonsense selected for response integration by \caps{Crest-e}.}
%     \label{fig:results-by-cstype}
% \end{figure*}




% We can also compare the rates between two approaches to gain insight about which characteristics are more influential to specific approaches. From this perspective, a large difference in the rates of some characteristic indicates that that characteristic is more of a determining factor behind the selection of responses from the model with the higher rate.

% Compared to Doctor, \caps{Crest-E} has a vastly higher rate of being preferred due to supportive, empathetic, and helpful response characteristics, and a slightly higher rate of being preferred on the basis of response detail. On the other hand, Doctor has a higher rate of responses being preferred due to their engagingness, positivity, and proactivity. Although Table \ref{tab:pairwise-comparisons} reveals that \caps{Crest-E} outperforms Doctor in terms of response engagingness, the engagingness of the Doctor responses is identified as a major contributing factor in the cases where Doctor is the preferred response in overall quality, more so than for \caps{Crest-E} relatively speaking.

% Notably, it can also be seen that a preference for \caps{Crest} responses is associated with specificity and supportiveness of the responses at a higher relative rate than the alternative approaches. In addition, the \caps{Crest} approach also is frequently preferred due to its tendency to display a high degree of empathy for the person being talked to, unlike the alternative approaches which have less indication that empathy is a contributing factor to overall performance. Additionally, the inclination of the responses to provide helpful advice and solutions to the events going on in the person's life also are unique characteristics that impact the \caps{Crest} approach more so than the other approaches.

% On the other hand, ChatGPT is most often explained as a preference due to the engagingness of the responses, and at a higher relative rate than that observed for \caps{Crest} or Doctor. In addition, responses from ChatGPT and Doctor are more frequently explained as being preferred due to their naturalness or their relevance to the context, relative to \caps{Crest}, although overall such characteristics are not a common explanation of preference.

==> section/old/results-tables.tex <==
\begin{table*}[htb]
    \centering
    \begin{tabular}{c|rrrr|rr}
        \toprule 
        & \multicolumn{2}{c}{\textbf{\caps{Crest}}} & \multicolumn{2}{c|}{\textbf{Doctor}} & \multirow{2}{*}{\textbf{\caps{Crest}}} & \multirow{2}{*}{\textbf{Doctor}} \\ 
        & Definitely & Slightly & Slightly & Definitely & & \\        \midrule 
        natural & 63.3 & 19.3 & 3.7 & 13.7 & 82.7 & 17.3 \\ 
        engaging & 74.0 & 18.3 & 2.7 & 5.0 & 92.3 & 7.7 \\ 
        specific & 69.7 & 21.7 & 3.3 & 5.3 & 91.3 & 8.7 \\ 
        quality & 68.7 & 23.3 & 2.3 & 5.7 & 92.0 & 8.0 \\ 
        \bottomrule 
    \end{tabular} 
    \caption{Pairwise evaluation results for \caps{Crest} vs Doctor showing the fine-grained preference selections by confidence level (left) and by overall sum (right). Overall sum for \caps{Crest} is statistically significant for all characteristics (proportion test, $\alpha < 0.01$).} 
    \label{tab:Crest-vs-Doctor} 
\end{table*}

\begin{table*}[htb]
    \centering
    \begin{tabular}{c|rrrr|rr}
        \toprule 
        & \multicolumn{2}{c}{\textbf{\caps{Crest}}} & \multicolumn{2}{c|}{\textbf{ChatGPT}} & \multirow{2}{*}{\textbf{\caps{Crest}}} & \multirow{2}{*}{\textbf{ChatGPT}} \\ 
        & Definitely & Slightly & Slightly & Definitely & & \\        \midrule 
        natural & 52.3 & 23.3 & 9.7 & 14.7 & 75.7 & 24.3 \\ 
        engaging & 52.3 & 30.3 & 8.3 & 9.0 & 82.7 & 17.3 \\ 
        specific & 56.3 & 30.0 & 6.0 & 7.7 & 86.3 & 13.7 \\ 
        quality & 55.3 & 29.0 & 8.0 & 7.7 & 84.3 & 15.7 \\ 
        \bottomrule 
    \end{tabular} 
    \caption{Pairwise evaluation results for \caps{Crest} vs ChatGPT showing the preference selections by confidence level (left) and by overall sum (right). Overall sum for \caps{Crest} is statistically significant for all characteristics (proportion test, $\alpha < 0.01$).} 
    \label{tab:Crest-vs-ChatGPT} 
\end{table*}

\begin{table*}[htb]
    \centering
    \begin{tabular}{c|rrrr|rr}
        \toprule 
        & \multicolumn{2}{c}{\textbf{ChatGPT}} & \multicolumn{2}{c|}{\textbf{Doctor}} & \multirow{2}{*}{\textbf{ChatGPT}} & \multirow{2}{*}{\textbf{Doctor}} \\ 
        & Definitely & Slightly & Slightly & Definitely & & \\        \midrule 
        natural & 56.0\% & 16.0\% & 7.3\% & 20.7\% & 72.0\% & 28.0\% \\ 
        engaging & 56.3\% & 26.0\% & 8.7\% & 9.0\% & 82.3\% & 17.7\% \\ 
        specific & 52.0\% & 25.7\% & 8.0\% & 14.3\% & 77.7\% & 22.3\% \\ 
        quality & 59.3\% & 21.3\% & 6.0\% & 13.3\% & 80.7\% & 19.3\% \\ 
        \bottomrule 
    \end{tabular} 
    \caption{Pairwise evaluation results for ChatGPT vs Doctor showing the fine-grained preference selections on the left and the total win percentages on the right.} 
    \label{tab:ChatGPT-vs-Doctor} 
\end{table*}
